Geometric averaging operators and nonconcentration inequalities

This paper is devoted to a systematic study of certain geometric integral inequalities which arise in continuum combinatorial approaches to $L^p$-improving inequalities for Radon-like transforms over polynomial submanifolds of intermediate dimension. The desired inequalities relate to and extend a number of important results in geometric measure theory.

==> header.tex <==
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{amsbsy}
\usepackage{amssymb}
\usepackage[initials]{amsrefs}
%\usepackage{epic}
%\usepackage{eepic}
%\usepackage{pstricks}
%\usepackage[mathscr]{eucal}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}

\newcommand{\R}{{\mathbb R}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\X}{{\mathfrak X}}
\newcommand{\Y}{{\mathfrak Y}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\Cminus}{{\cal C}}
\newcommand{\D}{{\cal D}}
\newcommand{\s}{{\cal S}^\infty}
\newcommand{\deriv}[1]{\partial_{#1}}
\newcommand{\ip}[2]{\left< #1, #2 \right>}
%\newcommand{\e}[2]{e^{-2 \pi i \left< #1, #2 \right>}}
\newcommand{\FT}{{\cal F}_z}
\newcommand{\F}{{\cal F}}
\newcommand{\real}[1]{\mathop{\mathrm{Re}}(#1)}
\newcommand{\imaginary}[1]{\mathop{\mathrm{Im}}(#1)}
\newcommand{\zp}{-Q-z}
\newcommand{\sip}[2]{ #1 \cdot #2}
\newcommand{\set}[2]{ \left\{ #1 \ \left| \ #2 \right. \right\} }
\newcommand{\CS}{Cauchy-Schwartz }
\newcommand{\supp}{\mathop{\mathrm{supp}}}
\newcommand{\vol}{\mbox{vol}}
\newenvironment{remark}
        {\textbf{Remark}}
        {\paragraph{}}

\newcommand{\ddt}{\frac{\partial}{\partial t}}
\newcommand{\ord}{\mathop{\mbox{ord}}}
\newcommand{\eX}{e^{\sum_{i,j} s_{i,j} X_{i,j}}}
\newcommand{\eY}{e^{tY_1}}
\newcommand{\dx}{{d_X}}
\newcommand{\dy}{{d_Y}}
\newcommand{\vspan}{\mathop{\mbox{span}}}
\newcommand{\all}{(M,X,Y,\pi_X,\pi_Y)}
\newcommand{\hint}[1]{[Hint: #1]}

